DatasetGAN: Efficient Labeled Data Factory with Minimal Human Effort

We introduce DatasetGAN: an automatic procedure to generate massive datasets of high-quality semantically segmented images requiring minimal human effort. Current deep networks are extremely data-hungry, benefiting from training on large-scale datasets, which are time consuming to annotate. Our method relies on the power of recent GANs to generate realistic images. We show how the GAN latent code can be decoded to produce a semantic segmentation of the image. Training the decoder only needs a few labeled examples to generalize to the rest of the latent space, resulting in an infinite annotated dataset generator! These generated datasets can then be used for training any computer vision architecture just as real datasets are. As only a few images need to be manually segmented, it becomes possible to annotate images in extreme detail and generate datasets with rich object and part segmentations. To showcase the power of our approach, we generated datasets for 7 image segmentation tasks which include pixel-level labels for 34 human face parts, and 32 car parts. Our approach outperforms all semi-supervised baselines significantly and is on par with fully supervised methods, which in some cases require as much as 100x more annotated data as our method.

==> doc/4_exp_s.tex <==
\vspace{-2mm}
\section{Experiments}{}
\label{sec:experiments}
\vspace{-1mm}

We extensively evaluate our approach. First, we perform evaluation on part segmentation across five different categories: Car, Face, Bird, Cat, and Bedroom(scene). Furthermore, we also label two keypoint datasets (Car and Bird), and also evaluate keypoint detection performance supported by our approach.  We finally showcase a qualitative 3D application that leverages our synthesized data for Car, to achieve single-image 3D asset creation. 

{\bf StyleGAN models:} Each class requires a pretrained category-specific StyleGAN model. For Car, Cat, Face and Bedroom, we directly use the pretrained StyleGAN models from the official GitHub repository provided by StyleGAN authors.  For bird, we train our own StyleGAN models on NABirds~\cite{7298658}, which contains 48k images.  
%Each class requires a category-specific StyleGAN model. We use the Car, Cat, Face, and Bedroom models from the official  StyleGAN repo. We also train a Bird model on NABirds~\cite{7298658}, which contains 48k images. 

\vspace{-2mm}
\subsection{Parts Segmentation} 
\label{sec:parts_result}

\vspace{-1mm}
\paragraph{Our Generated Datasets: } 
%We generate massive image and anntatoion pairs for each category. 
Figures~\ref{fig:vis_testing_cars},~\ref{fig:vis_testing2} show samples of synthesized image-annotation pairs for all classes used in the paper. We notice that higher resolution StyleGAN models (Bird, Face) result in more accurate synthesized annotations.  We provide more examples in the Appendix. 


\begin{figure}
\vspace{-4.5mm}
\begin{minipage}{0.62\linewidth}
\includegraphics[width=1\linewidth, trim=5 0 0 0,clip]{figs/num_data_vs_iou}
\end{minipage}
\hspace{1.5mm}
\begin{minipage}{0.32\linewidth}
\caption{\footnotesize\textbf{Number of training examples vs. mIOU}. We compare to baselines on ADE-Car-12 testing set. The red dash line represents the fully supervised method which exploits 2.6k training examples from ADE20k. }	
\label{fig:num_vs_iou}
\end{minipage}
\vspace{-6.5mm}
\end{figure}


% \begin{table*}[t!]
% \vspace{-1mm}
% \begin{center}
% \begin{minipage}{0.705\linewidth}
%  \begin{adjustbox}{width=1\linewidth}
% {\small
% \addtolength{\tabcolsep}{-2.5pt}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
% \hline
% Testing Dataset & ADE-Car-12 & ADE-Car-5 &  Car-20 & CelebA-Mask-8 (Face)  &   Face-34 & Bird-11 & Cat-16 & Bedroom-19  \\
% \hline 
% Num of Training Images & 	16     & 16             &16        & 16               & 16         & 30       & 30       & 40  \\ 
% \hline
% Num of Classes  & 12           & 5             & 20 &  8 & 34  &  11 & 16 &   19 \\ 
% \hline
% \hline
% Transfer-Learning& 24.04      & 45.16              & 36.62 &  62.66 &  44.83  & 22.58 & 20.35 & 24.74  \\ 
% \hline
% Transfer-Learning (\textbf{*})& 27.48      & 45.48              & \ding{55} &  64.56 &  \ding{55}  & \ding{55} & \ding{55} & \ding{55}  \\ 
% \hline
% Semi-Supervised~\cite{mittal2019semi} & 31.29 &  48.64 & 45.38 &  66.24& 46.99  &27.68  &27.35 &  34.64 \\ 
% \hline
% Semi-Supervised~\cite{mittal2019semi} (\textbf{*}) & 32.38 &  50.29   & \ding{55} &66.86 &  \ding{55}  & \ding{55} & \ding{55} & \ding{55}    \\ 
% \hline
% Ours  & \textbf{45.96}  &  \textbf{57.61} &  \textbf{63.01} & \textbf{71.10}  & \textbf{53.44}  & \textbf{36.72} &  \textbf{31.36} & \textbf{41.52}  \\ 
% \hline

% \end{tabular}\\
% }
% \end{adjustbox}
% {\scriptsize \ding{55} means that the method does not apply to this setting due to missing labeled data in the domain.}
% \end{minipage}
% \hfill
% \begin{minipage}{0.28\linewidth}
% \vspace{-1mm}
% \caption{\footnotesize {\bf Comparisons on Part Segmentation}.  \textbf{(*)} denotes In-domain experiment, where training and testing are conducted on the same dataset but a different split. Otherwise, training is conducted on our generated images. Note that In-domain setting does not apply to our approach, as we do not train StyleGAN on the provided datasets.} 
% \label{tbl:all_results}
% \end{minipage}
% \end{center}
% \vspace{-2.5mm}
% \end{table*}

\begin{table*}[t!]
\vspace{-1mm}
\begin{center}
\begin{minipage}{0.705\linewidth}
 \begin{adjustbox}{width=1\linewidth}
{\small
\addtolength{\tabcolsep}{-2.5pt}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
Testing Dataset & ADE-Car-12 & ADE-Car-5 &  Car-20 & CelebA-Mask-8 (Face)  &   Face-34 & Bird-11 & Cat-16 & Bedroom-19  \\
\hline 
Num of Training Images & 	16     & 16             &16        & 16               & 16         & 30       & 30       & 40  \\ 
\hline
Num of Classes  & 12           & 5             & 20 &  8 & 34  &  11 & 16 &   19 \\ 
\hline
\hline
Transfer-Learning& 24.85     &  44.92 & 33.91 $\pm$ 0.57  & 62.83 & 45.77 $\pm$ 1.51   & 21.33 $\pm$ 1.32    & 21.58 $\pm$ 0.61  & 22.52 $\pm$ 1.57   \\ 
\hline
Transfer-Learning (\textbf{*})& 29.71       &  47.22     & \ding{55} & 64.41  &  \ding{55}  & \ding{55} & \ding{55} & \ding{55}  \\ 
\hline
Semi-Supervised~\cite{mittal2019semi} & 28.68  & 45.07  & 44.51 $\pm$ 0.94  & 63.36 &48.17 $\pm$ 0.66  & 25.04 $\pm$ 0.29   &24.85 $\pm$ 0.35   & 30.15 $\pm$ 0.52   \\ 
\hline
Semi-Supervised~\cite{mittal2019semi} (\textbf{*}) & 34.82 & 48.76    & \ding{55} & 65.53 &  \ding{55}  & \ding{55} & \ding{55} & \ding{55}    \\ 
\hline
Ours  & \textbf{45.64}  &  \textbf{57.77} &  \textbf{62.33 $\pm$ 0.55} & \textbf{70.01}  & \textbf{53.46 $\pm$ 1.21}  & \textbf{36.76 $\pm$ 2.11} &  \textbf{31.26 $\pm$ 0.71 } & \textbf{36.83 $\pm$ 0.54}  \\ 
\hline

\end{tabular}\\
}
\end{adjustbox}
{\scriptsize \ding{55} means that the method does not apply to this setting due to missing labeled data in the domain.}
\end{minipage}
\hfill
\begin{minipage}{0.28\linewidth}
\vspace{-1mm}
\caption{\footnotesize {\bf Comparisons on Part Segmentation}.  \textbf{(*)} denotes In-domain experiment, where training and testing are conducted on the same dataset but a different split. Otherwise, training is conducted on our generated images. Note that In-domain setting does not apply to our approach, as we do not train StyleGAN on the provided datasets.} 
\label{tbl:all_results}
\end{minipage}
\end{center}
\vspace{-2.5mm}
\end{table*}



\begin{table*}[t!]
\vspace{-4mm}
\begin{minipage}{0.71\linewidth}
\begin{center}
 \begin{adjustbox}{width=1\linewidth}
{\scriptsize
\addtolength{\tabcolsep}{-3.5pt}
\begin{tabular}{l|c|c|c|c||c|c|c|c}
\hline
Testing Dataset &  \multicolumn{4}{c}{Car-20}  &   \multicolumn{4}{c}{CUB-Bird}  \\
\hline
Metric &  L2 Loss $\downarrow$ &  PCK th-15  $\uparrow$ &  PCK th-10  $\uparrow$    &  PCK th-5  $\uparrow$  & L2 Loss$\downarrow$	 &  PCK th-25  $\uparrow$   &  PCK th-15   $\uparrow$     &  PCK th-10  $\uparrow$  \\
\hline
Transfer Learn. &  4.4 $\times 10^{-4}$	 &  43.54  &  36.66     &  18.53 &  5.3 $\times 10^{-4}$&  23.17	 &  18.21   &  12.74    \\ 

Ours &  2.4 $\times 10^{-4}$	 &  79.91    &  67.14   &   35.17 &  4.3 $\times 10^{-4}$ & 60.61  &  46.36   &  32.00     \\ 
\hline
Fully Sup. &  \ding{55}	 &  \ding{55}   &  \ding{55}   &   \ding{55} &  3.2 $\times 10^{-4}$ & 77.54  & 65.00   &  53.73     \\ 

\hline

\end{tabular}   
}
\end{adjustbox}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{0.28\linewidth}
\caption{\footnotesize {\bf Comparisons on Keypoint Detection}.  Our method leads to significantly better results than those obtained by baseline methods. }
%\SF{say something about supervised?}}
%\ding{55} means that the method does not apply, due to the missing labeled data in the domain.} 
\label{tbl:Keypoints_result}
\end{minipage}
\vspace{-3mm}
\end{table*}


\vspace{-3.5mm}
\paragraph{Parts Segmentation Network:}  
For simplicity, we exploit Deeplab-V3~\cite{chen2017deeplab}, with ImageNet pre-trained ResNet151~\cite{he2016deep} backbone, as the part segmentation network to be trained on our synthesized datasets. We let Deeplab-V3 output one probability distribution over all part labels for each pixel. While exploiting part hierarchies in the model is possible, we opted for the simplest approach here. We use Deeplab-V3 as the backbone for all the baseline models.
%and we train the network using the Cross Entropy loss and Adam~\cite{adam} optimizer with learing rate 0.001. 

\vspace{-3.5mm}
\paragraph{Baselines:}   We compare our method to two types of baselines: Transfer-Learning and Semi-Supervised baseline. For the Transfer-Learning baseline, we initialize the network with the pre-trained weights on semantic segmentation of MS-COCO~\cite{Lin2014MicrosoftCC}, and finetune the last layer on our small human-annotated dataset in a supervised way. This baseline evaluates the standard practice in computer vision of pre-training on a large dataset  and only finetuning in-domain. It does not access unlabeled data on the target domain, but leverages a large labeled dataset from another domain. 
% Experimentally, since the pre-trained weights are not trained on parts segmentation task, we notice that the baseline works the best when we do not freeze any CNN weights.
We adopt~\cite{mittal2019semi} as the state-of-the-art semi-supervised baseline, and use the same pre-trained backbone as in our approach. We train this method on our human-labeled images plus the unlabeled \emph{real} images that the StyleGAN is trained on.  To demonstrate the effectiveness of our method, we further compare to a fully supervised baseline which is trained on a large number of labeled real images. Further details are in Appendix.  We emphasize that all methods and our approach use the same network architecture, and the only difference is the training data and algorithm. 

\vspace{-3.5mm}
\paragraph{Test Datasets:}  
For cars, we evaluate our model on part segmentation at different level of details, to leverage the existing datasets for benchmarking. Car instances from ADE20K~\cite{zhou2016semantic,zhou2017scene} and PASCAL~\cite{Everingham10} have 12 and 5 part labels, respectively.  We split cars in ADE20K testing set into our validation and testing sets, which contains 50 and 250 images. 
% We always crop instances by square bounding boxes with 15\% padding.
% In ADE20K, there are 2600 and 300 cars in training and testing split, respectively. 
We refer to cars from ADE20K as \textbf{ADE-Car-12} and further merge  labels from ADE-Car-12 into 5 classes (\textbf{ADE-Car-5}) according to the PASCAL annotation protocol.  We also exploit 900 cars from PASCAL for cross-domain testing purposes (no training), namely \textbf{PASCAL-Car-5}. For faces, we evaluate our model on CelebA-Mask-8~\cite{liu2015faceattributes}, which contains 30K images with 8 part categories. We exploit first 500 images in testing set as validation set. 
Since there is no existing fine-detailed part segmentation datasets for cat, bird, and bedrooms and both ADE-Car-12 and CelebA-Mask-8 are relatively coarse compared to our annotation, we manually annotate 20 test images for each category to evaluate the performance on detailed part labeling (described as ``Real" in Sec~\ref{sec:annotations}). We refer to them as~\textbf{Car-20},~\textbf{Face-34},~\textbf{Bird-11},~\textbf{Cat-16},~\textbf{Bedroom-19}, respectively.  We select images for these small test datasets from Stanford Cars~\cite{KrauseStarkDengFei-Fei_3DRR2013}, Celeb-A mask~\cite{liu2015faceattributes}, CUB~\cite{cub}, and Kaggle Cat~\cite{kaggle_cat}, respectively. For bedrooms, we pick 20 images from the web. A summary of all test datasets is in Table~\ref{tbl:all_results}.  Since there is no validation set for our annotated datasets, we splits testing images into five folds. We set each fold as validation and choose checkpoints accordingly. We report mean IOU and standard deviation.  


\begin{table*}[h!]

\begin{minipage}{.45\linewidth}
\begin{center}
{\footnotesize
\addtolength{\tabcolsep}{-0pt}
\begin{tabular}{|l|c|c|c|c|}
\hline
Generated Dataset Size & 3K & 5K & 10K & 20K \\ 
\hline
mIOU &  43.34 & 44.37  &   44.60 &  {\bf 45.04} \\
\hline
\end{tabular}   
\caption{\footnotesize {\bf Ablation study of synthesized dataset size.} Here, Style-Interpreter is trained on 16 human-labeled images.  Results are reported on ADE-Car-12 test set. Performance is slowly saturating. } 
\label{tbl:number_data}
}
\end{center}
\end{minipage}
\hspace{2mm}
\begin{minipage}{.535\linewidth}
\begin{center}
{\footnotesize
\addtolength{\tabcolsep}{-0pt}
\begin{tabular}{|l|c|c|c|c|}
\hline
Filtering Ratio & 0\% & 5\% & 10\% & 20\% \\ 
\hline
mIOU &  44.60 & 44.89  &   \textbf{45.64}  & 45.18 \\
\hline
\end{tabular}   
\caption{\footnotesize {\bf Ablation study of the filtering ratio.} We filter out the most uncertain synthesized Image-Annotation pairs.  Result shown are reported on ADE-Car-12 test set, using the generated dataset of size 10k. We use $10\%$ in other experiments.} 
\label{tbl:uncertainty_denoise}
}
\end{center}
\end{minipage}
\begin{minipage}{.45\linewidth}
\begin{center}
 \begin{adjustbox}{width=0.87\linewidth}
{\footnotesize
\addtolength{\tabcolsep}{-2.5pt}
\begin{tabular}{|l|c|c|c|}
\hline
Testing Dataset &  ADE-Car-5  & PASCAL-Car-5 \\
\hline
Num of Classes & 	5             & 5      \\
\hline
\hline
Deeplab-V3~\cite{chen2017deeplab}  (2600 labels)  &  59.41 (\textbf{*})             & 54.31  \\ 
\hline
Ours (25 labels)  &  57.71 &   55.65  \\ 
\hline
\end{tabular}   
}
\end{adjustbox}
\caption{\footnotesize {\bf Comparisons to fully supervised methods for Part Segmentation. } \textbf{(*)} denotes In domain experiments. Deeplab-V3 is trained on ADE-CAR and our model is trained on our generated dataset.  } 
\label{tbl:coarse_car_cross_domain}
\end{center}
\end{minipage}
\hspace{2mm}
\begin{minipage}{.535\linewidth}
\begin{center}
 \begin{adjustbox}{width=0.92\linewidth}
{\footnotesize
\addtolength{\tabcolsep}{-2.5pt}
\begin{tabular}{|l|c|c|c|c|}
\hline
Number of Annotated Images  & 1  & 7  &  13 & 19 \\ 
\hline 
Random &  25.63 $\pm$ 8.42 & 40.06 $\pm$ 1.32 & 42.44 & 44.41 \\
\hline
Active Learning &   33.93 & 40.88   &  43.49 & 46.82 \\
\hline
Manual &  33.92 & 41.19 &  43.61 & 46.74 \\
\hline
\end{tabular}  
}
\end{adjustbox} 
\caption{\footnotesize {\bf Data selection.} We compare different strategies for selecting StyleGAN images to be annotated by human.  mIoU is reported on ADE-Car-12 test set.  Mean and var over 5 runs are reported for random selection with 1 and 7 training examples.} 
\label{tbl:AL}
\end{center}
\end{minipage}
\vspace{-5mm}
\end{table*}

\vspace{-3.5mm}
\paragraph{Quantitative Comparison:}
We first compare our approach to Transfer-Learning and Semi-supervised baselines in Tab~\ref{tbl:all_results}. %All the baselines are trained with the same network architecture but different training datasets. 
We evaluate in both out-of-domain and in-domain settings, where baselines are trained on our annotated images (Sec.~\ref{sec:annotations}) or an equal number of randomly selected in-domain images (ADE cars). Note that our method falls in the out-of-domain setting, since we only train on our synthesized dataset and test on real images. Our method outperforms both Transfer-Learning and Semi-Supervised learning baselines on all classes by a large margin. Strikingly, on ADE-Car-12, our model outperforms the out-of-domain baselines by 20.79\% for Transfer-Learning and 16.96\% for Semi-supervised Learning, and outperforms two in-domain baselines by 15.93\% and 10.82\%, respectively. 

We further show the number of training images in our labeled datasets v.s mIOU and compare to baselines on ADE-Car-12 test set in Fig.~\ref{fig:num_vs_iou}. The red dash line is the fully supervised model trained on the full ADE-Car-12 training set (2600 images). Our approach, using the same architecture and hyperparameters, comparable with the fully supervised model with as few as \textbf{25} annotations, which is less than 1\% of what the fully supervised method uses. Finally, we show a comparison to fully supervised baseline on ADE-Car-5 and PASCAL-Car-5 in Table~\ref{tbl:coarse_car_cross_domain}. Here, our performance is not better than the fully supervised baseline on ADE-Car-5. We hypothesize this is due to ADE20K being out-of-domain for our model, and in-domain for the baseline, and that 2500 labeled examples used by the baseline are sufficient to train a good model for this easier 5-class task. 
Note that we outperform the baseline by 1.3\% when  both our models are evaluated in the out-of-domain setting on PASCAL-Car-5, showcasing better generalization capabilities. 





% \begin{table*}[t!]
% \begin{center}
% {\footnotesize
% \addtolength{\tabcolsep}{-2.5pt}
% \begin{tabular}{|l|c|c|c|}
% \hline
% Testing Dataset &  Coarse-CAR  & PASCAL-Car-5 \\
% \hline
% Num of Classes & 	5             & 5      \\
% \hline
% Deeplab-V3~\cite{chen2017deeplab}  (2600 data)  &  59.41 (\textbf{*})             & 54.31  \\ 
% \hline
% Our (25 data)  &  57.71 &   55.65  \\ 
% \hline
% \end{tabular}   
% \caption{\footnotesize {\bf Comparions to fully supervised methods for Parts Segmentation Task. }  \textbf{*}: In domain experiments. Reported Deeplab-V3 is trained on ADE-CAR and our model is trained on our generated dataset.} 
% \label{tbl:all_results}
% }
% \end{center}


% \end{table*}






\vspace{-3.5mm}
\paragraph{Ablation Studies:}
We ablate choices in our  approach on the Car category. We first ablate the size of generated dataset in Table~\ref{tbl:number_data}. Increasing the number of synthesized examples from 3,000 to 10,000 improves performance, however the improvement is marginal when we further add more data. We use the uncertainty denoising strategy described in Sec.~\ref{sec:factory} and report results of filtering the most uncertain examples using different ratios. As shown in Table~\ref{tbl:uncertainty_denoise}, denoising plays an important role. Removing noisy data is the result of a trade-off between diversity and uncertainty. Removing more uncertain (noisy) data means less diversity during training.  In experiments hereon, we set the size of the generated dataset to be 10,000 and filter out the top 10\% uncertain examples. 

\vspace{-3.5mm}
\paragraph{Training Data Selection:}
\label{sec:al_result}
In our approach, as few as \textbf{20} training examples are required for achieving good accuracy, which is remarkable for this level of detail. In such a low-data regime, selecting the right images to be manually labeled is crucial. We ablate three different options. The most straightforward selection protocol is to simply choose the images  randomly from the generated dataset. A more time consuming option, but one that is typically used when collecting datasets, is to 
employ a human (CV expert) to look through the dataset and select the most representative and diverse examples. Finally, as a more advanced strategy, active learning (AL) can be used, 
where selection and model training (training Style Interpreter) alternate in a continuous loop.  
Similarly to~\cite{Kuo2018CostSensitiveAL}, we exploit ensemble-based AL strategy~\cite{8579074} followed by applying coreset~\cite{Sener2017AGA}. We reuse the ensembles and JS divergence as described in Sec.~\ref{sec:factory} to calculate image uncertainty. We filter out the top k\% most uncertain examples and run coreset with $N$ centers on the top $k + 10 \%$ to $k \%$ percent of data to select the most representative examples. We use $N=12$ and $k=10$ in this paper. Finally, we ask our CV expert to select the top 6 most realistic images to be annotated out of the subset.

We compare these strategies in Table~\ref{tbl:AL}. In our experiment, in each round AL selects 6 training examples and we use mean of 10k random samples as the first example. Both manual and AL outperform random sampling. We also report standard deviation of the random selection (RS) strategy on 1 and 7 training examples, computed over 5 rounds. Upper bound performance of RS is similar to AL or the manual strategy. Note that AL requires re-labeling each time an experiment is run, and thus is not practical for the remainder of the paper. We instead exploit the manual selection strategy. 






\vspace{-3.5mm}
\paragraph{Qualitative Results:}
We showcase qualitative results on our test datasets in Fig~\ref{fig:vis_testing}. While not perfect, the results demonstrate that our approach leads to the labeling outputs of impressive quality, especially for operating in the few-shot regime. Most errors occur for thin parts (wrinkles or bird legs) or parts without visual boundaries (cat neck). 
%on exhaustedly annotated detailed part.




% \begin{figure*}[t!]
% \begin{tabular}{ccccc}
% \end{tabular}
% \begin{tabular}{c}
% \hspace{-2mm}\includegraphics[width=1\linewidth, trim=0 0 0 0,clip]{figs/stylegan_dataset/stylegan_dataset} \\[-0.3mm]
% \end{tabular}
% \vspace{-3mm}
% \caption{\footnotesize Stylegan Dataset}
% \label{fig:stylegan_dataset}
% \vspace{-3mm}
% \end{figure*}


\newcommand\hh{1.18cm}
\newcommand\ww{1.315cm}
\begin{figure*}[t!]
\vspace{-0.5mm}
\addtolength{\tabcolsep}{-5.5pt}
\begin{tabular}{p{1.25cm}cccccccccccc}
\iffalse
{\scriptsize {\bf Cars} $\qquad$ 12  cls.} &
%1-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_12/1.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_12/1_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/1_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/4.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/4_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/4_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/26.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/26_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/26_comps.jpg} &
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/14.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/14_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_12/14_comps.jpg}\\
\fi
{\scriptsize {\bf Cars} $\qquad$  20  cls.} &
%2-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_20/5.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_20/5_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/5_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/2.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/2_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/2_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/3.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/3_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/3_comps.jpg} &
% 4
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/8.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/8_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_20/8_comps.jpg} \\
{\scriptsize {\bf Cars} $\qquad$  32  cls.} &
%3-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_32/0.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_32/0_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/0_comps.jpg} &
% 2
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_32/5.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/car_32/5_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/5_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/1.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/1_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/1_comps.jpg} &
%4
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/3.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/3_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/car_32/3_comps.jpg} \\
{\scriptsize {\bf Faces} $\qquad$  34  cls.} &
%4-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/face/16.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/face/16_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/16_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/9.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/9_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/9_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/3.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/3_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/3_comps.jpg} &
% 4
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/15.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/15_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/15_comps.jpg}\\
{\scriptsize {\bf Faces} $\qquad$ 34  cls.} &
%5-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/face/8.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/face/8_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/8_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/13.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/13_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/13_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/12.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/12_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/12_comps.jpg} &
%4
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/10.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/10_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/face/10_comps.jpg}\\
{\scriptsize {\bf Birds} $\qquad$ 11  cls.} &
%5-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/bird/0.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/bird/0_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/0_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 50,clip]{figs/testing_vis/bird/2.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 50,clip]{figs/testing_vis/bird/2_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 50,clip]{figs/testing_vis/bird/2_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/4.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/4_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/4_comps.jpg} &
%4 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/12.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/12_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bird/12_comps.jpg}\\
{\scriptsize {\bf Cats} $\qquad$ 16  cls.} &
%6-1
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/cat/0.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/cat/0_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/0_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/2.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/2_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/2_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/7.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/7_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/7_comps.jpg} &
%4
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/11.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/11_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/cat/11_comps.jpg} \\[-1mm]

{\scriptsize {\bf Bedrooms} $\quad$ 19  cls.} &
\includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/bedroom/4.jpg} & \includegraphics[align=c,height=\hh,width=\ww, trim=0 0 0 0,clip]{figs/testing_vis/bedroom/4_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/4_comps.jpg} &
%2 
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/2.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/2_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/2_comps.jpg} &
%3
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/18.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/18_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/18_comps.jpg} &
%4
\includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/17.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/17_comps_gt.jpg} & \includegraphics[align=c,height=\hh,width=\ww,  trim=0 0 0 0,clip]{figs/testing_vis/bedroom/17_comps.jpg} \\[-1mm]


& {\scriptsize image} & {\scriptsize groundtruth} & {\scriptsize prediction} & {\scriptsize image} & {\scriptsize groundtruth} & {\scriptsize prediction} & {\scriptsize image} & {\scriptsize groundtruth} & {\scriptsize prediction} & {\scriptsize image} & {\scriptsize groundtruth} & {\scriptsize prediction} \\
\end{tabular}
\vspace{-1mm}
\caption{\footnotesize  {\bf Qualitative Results:} We visualize predictions of DeepLab trained on {\ours}'s datasets, compared to ground-truth annotations. Typical failure cases include parts that do not have clear visual boundaries (neck of the cat), or thin structures (facial wrinkles, bird legs, cat whiskers).}
\label{fig:vis_testing}
\vspace{-3mm}
\end{figure*}


\vspace{-1.5mm}
\subsection{Keypoint Detection} 
\label{sec:kp_result}
We showcase the generality of {\ours} by testing on another task, \ie keypoint detection. 

\vspace{-3.5mm}
\paragraph{Experimental Settings:}
We follow the common practice of keypoint detection, i.e. predicting heatmaps instead of keypoint locations. We apply the same strategy and settings as in the part segmentation experiments, except that the model outputs a heatmap per class instead of a probability distribution,  and L2 loss instead of cross-entropy loss is used.  Similarly, we compare our approach to the Transfer-Learning baseline on Car and Bird. We evaluate the bird model on the CUB bird dataset,  while the car model on 20 manually-labeled real images since no previous car dataset have keypoints annotation as fine as ours. 

\vspace{-5.5mm}
\paragraph{Results:}
Performance evaluation is reported on the test set in Table~\ref{tbl:Keypoints_result}, with qualitative results in Fig.~\ref{fig:vis_kp}. 
Results demonstrate that our approach significantly outperforms the fine-tuning baseline using the same annotation budget. 


\newcommand\hhh{0.95cm}
\newcommand\www{1.42cm}
\begin{figure*}[t!]
\vspace{-0mm}
\addtolength{\tabcolsep}{-5.5pt}
\begin{tabular}{cccccccccccc}
%\hspace{-2mm}\includegraphics[width=1\linewidth, trim=0 0 0 0,clip]{figs/keypoints/kp_results} \\[-0.3mm]
% 1-1
\includegraphics[align=c,height=\hhh,width=\www, trim=10 20 0 20,clip]{figs/keypoints/kp_pred_car/car_GT_1.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=10 20 0 20,clip]{figs/keypoints/kp_pred_car/car_PRED_1.png} &
%2
\includegraphics[align=c,height=\hhh,width=\www, trim=20 0 0 0,clip]{figs/keypoints/kp_pred_car/car_GT_2.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=25 0 0 0,clip]{figs/keypoints/kp_pred_car/car_PRED_2.png} &
%3
\includegraphics[align=c,height=\hhh,width=\www, trim=0 20 0 10,clip]{figs/keypoints/kp_pred_car/car_GT_3.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 20 0 10,clip]{figs/keypoints/kp_pred_car/car_PRED_3.png} &
%4
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 20,clip]{figs/keypoints/kp_pred_car/car_GT_7.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 20,clip]{figs/keypoints/kp_pred_car/car_PRED_7.png} &
%5
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 20,clip]{figs/keypoints/kp_pred_car/car_GT_4.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 20,clip]{figs/keypoints/kp_pred_car/car_PRED_4.png} &
%6
\includegraphics[align=c,height=\hhh,width=\www, trim=0 10 0 20,clip]{figs/keypoints/kp_pred_car/car_GT_9.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 10 0 20,clip]{figs/keypoints/kp_pred_car/car_PRED_9.png} \\
% 2-1
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_GT_22.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_Pred_22.png} &
%2
\includegraphics[align=c,height=\hhh,width=\www, trim=30 40 30 40,clip]{figs/keypoints/kp_pred_bird/bird_GT_5.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=30 40 30 40,clip]{figs/keypoints/kp_pred_bird/bird_Pred_5.png} &
%3
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_GT_9.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_Pred_9.png} &
%4
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_GT_0.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_Pred_0.png} &
%5
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_GT_18.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_Pred_18.png} &
%6
\includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_GT_14.png} & \includegraphics[align=c,height=\hhh,width=\www, trim=0 0 0 0,clip]{figs/keypoints/kp_pred_bird/bird_Pred_14.png} \\[-0.7mm]
{\scriptsize groundtruth}  & {\scriptsize prediction} & {\scriptsize groundtruth}  & {\scriptsize prediction} & {\scriptsize groundtruth}  & {\scriptsize prediction} & {\scriptsize groundtruth}  & {\scriptsize prediction}& {\scriptsize groundtruth}  & {\scriptsize prediction}& {\scriptsize groundtruth}  & {\scriptsize prediction}\\ 
\end{tabular}
\vspace{-1mm}
\caption{\footnotesize {\bf Quantitative results for Keypoint Detection}. \textbf{First row:} Model trained on the generated dataset using 30 human-provided annotations. Results shown are on CUB-Bird test set. \textbf{Second row:} Here 16 human-provided annotations are used.  Results shown are on Car-20 test set. }
\label{fig:vis_kp}
\vspace{-2mm}
\end{figure*}



% \begin{figure*}[t!]
% \vspace{-0mm}
% \centering
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_11_1.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_11_1.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_15_1.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_15_1.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_100_3.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_100_3.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_126_1.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_126_1.jpg}
% \end{minipage}
% \caption{\footnotesize {\bf 3D Application:} We showcase our part segmentation an keypoint detection in reconstructing 3D objects from images. }
% \label{fig:3d}
% \vspace{-2mm}
% \end{figure*}

% \begin{figure*}[t!]
% \vspace{-0mm}
% \centering
% \begin{minipage}[t!] {0.055\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_11_1.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_11_1.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.055\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_15_1.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_15_1.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.12\textwidth}
% \centering
% \includegraphics[width=\textwidth, trim=0 0 200 0,clip]{figs/3d/JF/view1.png}
% \end{minipage}
% \begin{minipage}[t] {0.055\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_100_3.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_100_3.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.055\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \includegraphics[width=\textwidth]{figs/3d/input/imview_11_1_ori_input.png}
% \end{minipage}
% \begin{minipage}[t] {0.37\textwidth}
% \centering
% \includegraphics[width=\textwidth,trim=0 700 0 180,clip]{figs/3d/imview_126_1.jpg}\\[-1mm]
% \includegraphics[width=\textwidth,trim=0 0 0 880,clip]{figs/3d/imview_126_1.jpg}
% \end{minipage}
% \begin{minipage}[t] {0.12\textwidth}
% \centering
% \includegraphics[width=\textwidth, trim=0 0 200 0,clip]{figs/3d/JF/view2.png}
% \end{minipage}
% \caption{\footnotesize {\bf 3D Application:} We showcase our part segmentation an keypoint detection in reconstructing 3D objects from images. }
% \label{fig:3d}
% \vspace{-2mm}
% \end{figure*}

\newcommand\hn{1.53cm}
\begin{figure*}[t!]
\vspace{-0.5mm}
\centering
\begin{minipage}[t!] {\textwidth}
\centering
\includegraphics[height=\hn]{figs/3d/input/imview_11_1_comb.png}
\includegraphics[height=\hn]{figs/3d/pred/imview_11_1.jpg}
\includegraphics[height=\hn]{figs/3d/input/imview_15_1_comb.png}
\includegraphics[height=\hn]{figs/3d/pred/imview_15_1.jpg}
\includegraphics[height=\hn]{figs/3d/JF/view1.png}
\end{minipage}
\begin{minipage}[t] {\textwidth}
\centering
\includegraphics[height=\hn]{figs/3d/input/imview_100_3_comb.png}
\includegraphics[height=\hn]{figs/3d/pred/imview_100_3.jpg}
\includegraphics[height=\hn]{figs/3d/input/imview_126_1_comb.png}
\includegraphics[height=\hn]{figs/3d/pred/imview_126_1.jpg}
\includegraphics[height=\hn]{figs/3d/JF/view2.png}
\end{minipage}
\caption{\footnotesize {\bf 3D Application:} We showcase our detailed part segmentation and keypoint detection in reconstructing animatable 3D objects from monocular images. We follow~\cite{zhang2020image} for training the inverse graphics network, but augment it with 3D part segmentation and 3D keypoint branches, which we supervise with 2D losses. Top left corner shows the input image, keypoint prediction is in the bottom, followed by a rendering of the predicted textured \& segmented 3D model into several views. We show an animated scene with lit front and back lights in the last column, which is made possible due to our 3D part segmentation. Cars have physics, rigged wheels, and can be driven virtually. See Supplementary for a video.}
\label{fig:3d}
\vspace{-3mm}
\end{figure*}



\vspace{-2mm}
\subsection{3D Application: Animatable 3D Assets}
\label{sec:3d}
\vspace{-2mm}
We now showcase how detailed part and keypoint prediction tasks can be leveraged in one downstream application. In particular, we aim to perform 3D reconstruction from single images (inverse rendering) to get rich 3D assets that can be animated realistically and potentially used in 3D games. This result is the first result of its kind. 

We focus on cars.  We aim to utilize the predicted keypoints as a way to estimate better 3D shape from monocular images. We further aim to map part segmentation to the estimated 3D model, which can then be used for post-processing: 1) placing correct materials for each part such as transparent windshields, 2) creating emissive lighting, and 3) replacing wheels with rigged wheels from an asset store, to enable the estimated 3D cars to drive realistically. 

%\vspace{-3mm}
%\paragraph{Details:}
We follow a similar pipeline as in~\cite{zhang2020image} to predict 3D shapes, texture, but also predict 3D parts and 3D keypoints. In particular, we first use StyleGAN to generate multiview images for different content codes. We then use our Style Interpreter to generate part  and keypoint labels. We train an inverse graphics network that accepts an image as input and predicts 3D shape, texture, 3D part labeling and 3D keypoints, by utilizing differentiable rendering~\cite{dib-r}. %Following practices in 3D literature~\cite{dib-r,softras,nmr}, we deform from a sphere to get the shape, and use fixed UV coordinates for the texture. 
%3D shape is parametrized as a deformed sphere. 
For 3D parts, we predict a part map, and paste it onto 3D shape (deformed sphere) in the same manner as for texture. For 3D keypoints, we learn a probability distribution over all vertices in the deformed shape.  We utilize all losses from~\cite{dib-r,zhang2020image}, and add an L2 loss on the projected keypoints, and Cross Entropy loss on the projected part segmentation. Details are in the Appendix. 

\vspace{-4mm}
\paragraph{Results:}
\vspace{-1.5mm}
We provide qualitative results in Fig.~\ref{fig:3d}, with additional results in Appendix, by highlighting the predicted part segmentation and animatable 3D assets. 
%We faithfullly reconstruct 3D geometry, texture, part segmentation and key points from single image. We further rendering the generated 3D shape by adding the light source to the front and back car lighs, this can further provide 3D assests for many applications, e.g. simulation. 




